An Audit on the Perspectives and Challenges of Hallucinations in NLP

We audit how hallucination in large language models (LLMs) is characterized in peer-reviewed literature, using a critical examination of 103 publications across NLP research. Through the examination of the literature, we identify a lack of agreement with the term `hallucination' in the field of NLP. Additionally, to compliment our audit, we conduct a survey with 171 practitioners from the field of NLP and AI to capture varying perspectives on hallucination. Our analysis calls for the necessity of explicit definitions and frameworks outlining hallucination within NLP, highlighting potential challenges, and our survey inputs provide a thematic understanding of the influence and ramifications of hallucination in society.

==> content/10_miscellaneous.tex <==
Miscellaneous ideas which can be part of the paper

1. Talk about Google's issue of hallucination during Bard release which decreased their stock value by 10\%
2. OpenAI openly admitting that their models hallucinate after 2-3 months of releasing ChatGPT in Nov 2022.
3. Increasing importance on guard-railing in industry during inference time for real-world AI applications

